Examining the Social Context of Alcohol Drinking in Young Adults with Smartphone Sensing

According to prior work, the type of relationship between the person consuming alcohol and others in the surrounding (friends, family, spouse, etc.), and the number of those people (alone, with one person, with a group, etc.) are related to many aspects of alcohol consumption, such as the drinking amount, location, motives, and mood. Even though the social context is recognized as an important aspect that influences the drinking behavior of young adults in alcohol research, relatively little work has been conducted in smartphone sensing research on this topic. In this study, we analyze the weekend nightlife drinking behavior of 241 young adults in Switzerland, using a dataset consisting of self-reports and passive smartphone sensing data over a period of three months. Using multiple statistical analyses, we show that features from modalities such as accelerometer, location, application usage, bluetooth, and proximity could be informative about different social contexts of drinking. We define and evaluate seven social context inference tasks using smartphone sensing data, obtaining accuracies of the range 75%-86% in four two-class and three three-class inferences. Further, we discuss the possibility of identifying the sex composition of a group of friends using smartphone sensor data with accuracies over 70%. The results are encouraging towards (a) supporting future interventions on alcohol consumption that incorporate users' social context more meaningfully, and (b) reducing the need for user self-reports when creating drink logs.

==> extras.tex <==


\begin{table}[t]
        \small
        \centering
        \caption{Social Context Inference accuracy breakdown for sensor type based feature groups and feature group combinations using Random Forest classifiers. Both the mean (\={A}) and standard deviation (A$_{\sigma}$) of accuracies from cross validation are reported in addition to the mean area under the curve (AUC) from reciever operator characteristics graph (ROC)}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{l l l l l l l l l l l l l l l l }

        \rowcolor{red!5}
        \textbf{Feature Group} & 
        \multicolumn{8}{c}{\textbf{two-class}} &
        &
        \multicolumn{6}{c}{\textbf{three-class}} 
        \\
        
        \arrayrulecolor{red!5} \specialrule{6pt}{0pt}{-6pt} \arrayrulecolor{black}
        \cmidrule{2-9}
        \cmidrule{11-16}
        
        \rowcolor{red!5}
        \textbf{(\# of features)}& 
        %\textbf{baseline} &
        \textbf{family$_{two}$} & 
        &
        \textbf{partner$_{two}$} & 
        &
        \textbf{friends$_{two}$} & 
        &
        \textbf{people$_{two}$}& 
        &
        &
        %\textbf{baseline} &
        \textbf{family$_{three}$} & &
        \textbf{friends$_{three}$} & &
        \textbf{people$_{three}$} &
        
        \\
        \rowcolor{red!5}
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        &
        \={A} (A$_{\sigma}$), AUC$_{S1}$, AUC$_{S2}$ & % baseline
        
        \\

        \hline 
        Baseline &
        50.0 (0.0), 50.0, 50.0& % baseline
        &
        50.0 (0.0), 50.0, 50.0& % 2 - family
        &
        50.0 (0.0), 50.0, 50.0& % 2 - partner
        &
        50.0 (0.0), 50.0, 50.0& % 2 - alone
        &
        &
        33.3 (0.0), 50.0, 50.0& % baseline
        &
        33.3 (0.0), 50.0, 50.0& % 3 - friends
        &
        33.3 (0.0), 50.0, 50.0&  % 3 - alone
        
        \\
        
        \iffalse
        DEM (50) &
        %50.00\% & % baseline
        74.4 & % 2 - family
        &
        70.2 & % 2 - partner
        &
        63.9 & % 2 - friends
        &
        61.1 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        61.9 & % 3 - family
        &
        60.5 & % 3 - friends
        &
        57.7 &  % 3 - alone
        
        \\
        \fi 
        
        
        ACC (150) &
        %50.00\% & % baseline
        83.3 (2.4), 80.2, 74.6 & % 2 - family
        &
        81.2 (3.1), 79.6, 71.1 & % 2 - partner
        &
        74.9 (3.0), 72.5, 68.3 & % 2 - friends
        &
        81.1 (3.1), 81.4, 69.8 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        82.6 (1.9), 78.5, 73.8 & % 3 - family
        &
        71.5 (2.5), 70.1, 69.4 & % 3 - friends
        &
        72.4 (2.7), 72.0, 69.9 &  % 3 - alone
        
        \\
        
        

        \rowcolor{gray!5}
        APP (105)&
        %50.00\% & % baseline
        82.9 (3.5), 80.7, 70.3 & % 2 - family
        &
        82.9 (3.0), 79.2, 71.1 & % 2 - partner
        &
        74.3 (2.4), 76.7, 68.6 & % 2 - friends
        &
        80.5 (2.5), 81.1, 70.1 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        81.4 (2.4), 81.5, 73.9 & % 3 - family
        &
        69.5 (3.1), 69.1, 68.3 & % 3 - friends
        &
        71.9 (2.3), 70.2, 69.1 &   % 3 - alone
    
        \\
        
        
        BAT (36)&
        %50.00\% & % baseline
        78.7 (2.8), 76.7, 66.7 & % 2 - family
        &
        77.5 (3.6), 77.3, 68.6 & % 2 - partner
        &
        71.5 (3.0), 73.6, 65.8 & % 2 - friends
        &
        78.1 (3.3), 72.1, 69.4 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        77.5 (2.7), 75.6, 71.6 & % 3 - family
        &
        66.1 (3.1), 67.8, 65.5 & % 3 - friends
        &
        68.1 (2.6), 68.4, 67.3 &   % 3 - alone

        \\
        
        \rowcolor{gray!5}
        BLU (27)&
        %50.00\% & % baseline
        74.6 (2.8), 72.1, 62.8 & % 2 - family
        &
        75.5 (3.6), 73.8, 62.1 & % 2 - partner
        &
        69.0 (2.8), 70.3, 59.7 & % 2 - friends
        &
        74.0 (3.1), 73.1, 65.5 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        69.3 (2.9), 68.8, 67.4 & % 3 - family
        &
        59.4 (2.7), 61.4, 59.9 & % 3 - friends
        &
        60.5 (2.8), 66.4, 62.1 &   % 3 - alone
        
        \\
        
        
        PRO (18)&
        %50.00\% & % baseline
        74.1 (3.1), 71.9, 62.2 & % 2 - family
        &
        75.6 (2.3), 74.5, 62.9 & % 2 - partner
        &
        69.9 (2.8), 68.2, 63.2 & % 2 - friends
        &
        75.8 (2.7), 76.8, 66.1 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        70.4 (2.2), 73.2, 66.3 & % 3 - family
        &
        59.1 (3.8), 61.9, 60.3 & % 3 - friends
        &
        60.7 (2.4), 62.9, 63.2 &   % 3 - alone
        
        \\
        

        \rowcolor{gray!5}
        LOC (39)&
        %50.00\% & % baseline
        79.2 (3.0), 77.1, 67.1 & % 2 - family
        &
        78.9 (2.7), 78.2, 67.2 & % 2 - partner
        &
        74.1 (3.2), 76.1, 66.9 & % 2 - friends
        &
        77.6 (2.6), 76.9, 71.0 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        77.2 (2.6), 76.4, 71.9 & % 3 - family
        &
        67.0 (3.3), 69.1, 66.1 & % 3 - friends
        &
        69.5 (2.9), 68.7, 68.5 &   % 3 - alone
        
        \\
        
        
        SCR (3) &
        %50.00\% & % baseline
        68.3 (4.5), 61.1, 55.2 & % 2 - family
        &
        69.7 (4.7), 60.3, 56.4 & % 2 - partner
        &
        64.5 (4.6), 62.8, 55.9 & % 2 - friends
        &
        71.9 (3.1), 67.2, 61.1 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        62.2 (5.6), 60.7, 59.9 & % 3 - family
        &
        54.1 (4.3), 55.2, 53.7 & % 3 - friends
        &
        54.8 (5.5), 56.1, 54.8 &  % 3 - alone
        
        \\
        

        \rowcolor{gray!5}
        WIF (36)&
        %50.00\% & % baseline
        77.5 (2.9), 78.1, 64.2 & % 2 - family
        &
        77.1 (2.9), 76.9, 66.1 & % 2 - partner
        &
        68.8 (3.7), 70.2, 63.4 & % 2 - friends
        &
        75.3 (3.9), 76.1, 64.5 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        73.1 (1.9), 73.0, 68.7 & % 3 - family
        &
        61.6 (2.9), 63.6, 62.3 & % 3 - friends
        &
        64.5 (2.8), 67.1, 62.6 &   % 3 - alone
        
        \\
        
        
        \cmidrule{2-9}
        \cmidrule{11-16}
        
        ConSen (306) &
        %50.00\% & % baseline
        85.7 (2.6), 82.1, 72.9 & % 2 - family
        &
        86.8 (2.9), 80.8, 74.5 & % 2 - partner
        &
        79.5 (3.2), 80.2, 73.1 & % 2 - friends
        &
        82.9 (2.1), 81.4, 74.8 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        85.3 (1.9), 76.8, 76.2 & % 3 - family
        &
        76.7 (2.7), 76.9, 73.1 & % 3 - friends
        &
        77.9 (3.0), 76.1, 73.6 &   % 3 - alone
        \\
        
        \iffalse
        \[ACC, BAT, BLU, WIF, LOC, PRO\] &
        %50.00\% & % baseline
         & % 2 - family
         &
         & % 2 - partner
         &
         & % 2 - friends
         &
         & % 2 - alone
        &
        &
        %33.33\% & % baseline
         & % 3 - family
         &
         & % 3 - friends
         &
         &  % 3 - alone
        
        \\
        \fi 

        \rowcolor{gray!5}
        IntSen (96) &
        %50.00\% & % baseline
        83.3 (2.0), 80.1, 70.8 & % 2 - family
        &
        83.1 (2.5), 81.7, 72.1 & % 2 - partner
        &
        76.5 (2.9), 76.3, 70.0 & % 2 - friends
        &
        81.6 (2.5), 81.5, 71.3 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        82.3 (2.7), 78.2, 74.4 & % 3 - family
        &
        71.4 (2.7), 71.2, 69.1 & % 3 - friends
        &
        73.2 (2.7), 72.7, 69.8 &   % 3 - alone
        
        \\
        
        \iffalse
        \rowcolor{gray!5}
        \[APP, SCR\] &
        & % 2 - family
        &
         & % 2 - partner
        &
         & % 2 - friends
        &
         & % 2 - alone
        & 
         &
         & % 3 - family
        &
         & % 3 - friends
        &
         & % 3 - alone
        
        \\
        \fi 
        
        %\specialrule{6pt}{0pt}{-6pt} %\arrayrulecolor{black}
        \cmidrule{2-9}
        \cmidrule{11-16}
        
        ALL (402) &
        %50.00\% & % baseline
        86.1 (3.1), 84.8, 81.5 & % 2 - family
        &
        87.4 (2.6), 82.6, 75.0 & % 2 - partner
        &
        80.1 (2.9), 81.3, 73.5 & % 2 - friends
        &
        83.3 (2.2), 79.2, 75.1 & % 2 - alone
        &
        &
        %33.33\% & % baseline
        85.9 (2.2), 80.5, 76.3 & % 3 - family
        &
        76.7 (2.3), 78.2, 73.2 & % 3 - friends
        &
        78.3 (2.1), 75.3, 73.8 &   % 3 - alone
        
        \\
        \hline 
        \end{tabular}}
        \label{tab:inference_results_v3}
\vspace{-0.2 in}
\end{table}




\begin{table}[t]
        \small
        \centering
        \caption{Mean (\={A}) and Standard Deviation (A$_{\sigma}$) of inference accuracies and the mean area under the curve of the receiver operator characteristic curve (AUC), calculated from 10 iterations, using five different models, for two-class and three-class tasks, with attributes such as family, friends/colleagues, spouse/partner, and alone. Results are presented as: \={A} (A$_{\sigma}$), AUC}
        \resizebox{0.77\textwidth}{!}{%
        \begin{tabular}{c l l l l l l}

        \rowcolor{red!5}
        &
        \textbf{Target Variable}& 
        \textbf{Random Forest} &
        \textbf{XG Boost} &
        \textbf{Ada Boost} &
        \textbf{Gradient Boost}&
        \textbf{Naive Bayes} 
        \\

        \hline 
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{\textbf{two-class}}}}&
        baseline &
        50.0 (0.0), 50.0 & % RF
        50.0 (0.0), 50.0 & % XGBoost
        50.0 (0.0), 50.0 & % AdaBoost
        50.0 (0.0), 50.0 & % GradientBoost
        50.0 (0.0), 50.0 % NaiveBayes
        \\
        
        
        &
        \rowcolor{gray!5}
        family$_{two}$  &
        \textbf{86.1} (3.1), 84.8 & % RF
        82.6 (3.4), 67.4 & % XGBoost
        82.5 (4.2), 68.2& % AdaBoost
        83.2 (3.7), 71.1 & % GradientBoost
        65.6 (6.9), 63.1 % NaiveBayes
        \\
        
        &
        partner$_{two}$  &
        \textbf{87.4} (2.6), 82.6 & % RF
        84.6 (4.6), 70.1 & % XGBoost
        83.5 (3.8), 67.4 & % AdaBoost
        84.7 (5.1), 71.7 & % GradientBoost
        68.6 (8.2), 61.8 % NaiveBayes
        \\
        
        &
        \rowcolor{gray!5}
        friends$_{two}$  &
        \textbf{80.1} (2.9), 81.3 & % RF
        78.3 (4.5), 71.6 & % XGBoost
        78.0 (4.1), 69.1 & % AdaBoost
        78.7 (3.7), 70.9 & % GradientBoost
        64.0 (4.2), 65.7 % NaiveBayes
        \\

        &
        people$_{two}$ &
        83.3 (3.2), 79.2 & % RF
        84.1 (3.1), 72.4 & % XGBoost
        82.7 (4.3), 67.2 & % AdaBoost
        \textbf{84.2} (2.8), 72.7 & % GradientBoost
        72.3 (4.7), 64.7  % NaiveBayes
        \\
        
        \cmidrule{2-7}
        
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\footnotesize{\textbf{three-class}}}}&
        \rowcolor{gray!5}
        baseline &
        33.3 (0.0), 50.0 & % RF
        33.3 (0.0), 50.0 & % XGBoost
        33.3 (0.0), 50.0 & % AdaBoost
        33.3 (0.0), 50.0 & % GradientBoost
        33.3 (0.0), 50.0 % NaiveBayes
        \\
        
        
        &
        family$_{three}$  &
        \textbf{85.9} (2.2), 80.5 & % RF
        81.4 (3.1), 68.3 & % XGBoost
        73.9 (3.7), 58.3 & % AdaBoost
        83.0 (2.6), 69.7 & % GradientBoost
        63.1 (4.2), 61.3 % NaiveBayes
        \\
        
        
        &
        \rowcolor{gray!5}
        friends$_{three}$  &
        76.7 (2.3), 78.2 & % RF
        77.1 (3.6), 68.3 & % XGBoost
        71.0 (3.1), 66.9& % AdaBoost
        \textbf{77.6} (2.8), 71.8 & % GradientBoost
        62.2 (5.1), 62.4 % NaiveBayes
        \\
        
        &
        people$_{three}$  &
        \textbf{78.3} (2.1), 75.3 & % RF
        71.2 (2.6), 69.5 & % XGBoost
        67.1 (3.8), 65.9 & % AdaBoost
        73.8 (3.2), 70.4 & % GradientBoost
        57.9 (6.7), 65.7 % NaiveBayes
        \\
        
        \hline 
        
        \end{tabular}}
        \label{tab:inference_results}

\end{table}


\begin{table}[t]
        \small
        \centering
        \caption{Sex-Composition Inference results for alcohol consumption episodes done with friends, in the order: \={A} (A$_{\sigma}$), AUC }
        \resizebox{0.85\textwidth}{!}{%
        \begin{tabular}{ l l l l l l}

        \rowcolor{red!5}
        
        \textbf{Target Variable}& 
        \textbf{Random Forest} &
        \textbf{XG Boost} &
        \textbf{Ada Boost} &
        \textbf{Gradient Boost}&
        \textbf{Naive Bayes} 
        \\

        \hline 
        
        baseline &
        33.3 (0.0), 50.0 & % RF
        33.3 (0.0), 50.0 & % XGBoost
        33.3 (0.0), 50.0 & % AdaBoost
        33.3 (0.0), 50.0 & % GradientBoost
        33.3 (0.0), 50.0 % NaiveBayes
        \\
        
        \rowcolor{gray!5}
        sex\_composition$_{three}$  &
        75.8 (2.5), 72.8 & % RF
        69.6 (4.1), 69.2 & % XGBoost
        66.1 (6.1), 65.8 & % AdaBoost
        71.5 (3.7), 70.3 & % GradientBoost
        58.7 (7.3), 58.9 % NaiveBayes
        \\
        
        
        \hline 
        
        \end{tabular}}
        \label{tab:inference_sex}
\vspace{-0.2 in}
\end{table}




\begin{table}[t]
    \centering
    \caption{Pearson Correlation Co-efficient (PCC) and Point-Biserial Correlation Co-efficient (PBCC) for Sensor Features and Social Contexts (two-class and three-class). Only the top 10 features for each Social Context are included in the table. p-values are denoted in the following notation: p-value\leq10$^{-4}$:****; p-value\leq10$^{-3}$:***; p-value\leq10$^{-2}$:**; p-value\leq10$^{-1}$:*}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l l  l l  l l  l l }
    
    \rowcolor{red!5}
    &
    \multicolumn{2}{c}{\textbf{family}}&
    \multicolumn{2}{c}{\textbf{partner}}&
    \multicolumn{2}{c}{\textbf{friends}}&
    \multicolumn{2}{c}{\textbf{alone}}
    \\
    
    \rowcolor{red!5}
    &
    \textbf{Feature (Sensor)} & 
    \textbf{PBCC} &
    \textbf{Feature (Sensor)} &
    \textbf{PBCC} &
    \textbf{Feature (Sensor)} & 
    \textbf{PBCC} &
    \textbf{Feature (Sensor)} &
    \textbf{PBCC} 
    \\
    \hline
    
    \multirow{10}{*}{\rotatebox[origin=c]{90}{\footnotesize{two-class}}}  &
    {angleXMax\_min (ACC)} & % family feature
    0.19 (+) **** &  % pearson
    
    {yAxisAvgMax\_avg (ACC)} &  % people feature
    {0.14 (-)} **** &  % pearson
    
    mMean\_avg (ACC) &  % partner feature
    0.22 (+) **** &  % point-biserial
    
    mMed\_max (ACC) & % friends feature
    {0.19} (+) ****  % pearson
    
    
    \\
    
    
    &
    {angleXMed\_min (ACC)} & % family feature
    {0.19 (+)} ****&  % pearson
    
    {food\_and\_drink\_avg (APP)} &  % people feature
    {0.13 (+)} *** & % pearson
    
    mSMAMean\_avg (ACC) &  % partner feature
    0.22 (+) ****&  % point-biserial
    
    mSMAMed\_max (ACC) & % friends feature
    0.19 (+) ****  % pearson
    
    
    \\
    
    &
    {angleYAvg\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    {food\_and\_drink\_min (APP)} &  % people feature
    {0.12 (+) ***} &  % pearson
    
    mMed\_max (ACC) &  % partner feature
    0.22 (+) **** &  % point-biserial
    
    mMean\_max (ACC) & % friends feature
    0.19 (+) ****   % pearson
    
    
    \\
    
    
    
    &
    {angleXAvg\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    {food\_and\_drink\_min (APP)} &  % people feature
    {0.12 (+) ***} &  % pearson
    
    mSMAMed\_max (ACC) &  % partner feature
    0.22 (+) ****&  % point-biserial
    
    mSMAMean\_max (ACC) & % friends feature
    0.19 (+) ****  % pearson
    
    
    \\
    
    &
    {angleYMax\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    {zAxisAvgMin\_avg (ACC)} &  % people feature
    {0.12 (+) ***} & % pearson
    
    mMax\_avg (ACC) &  % partner feature
    0.21(+) ****&  % point-biserial
    
    dmListStd\_max (ACC) & % friends feature
    0.18 (+) ****  % pearson
    
    
    \\
    
    &
    {angleYMed\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    {blueStrengthMin\_max (BLU)} &  % people feature
    {0.10 (-) ***} & % pearson
    
    mSMAMax\_avg (ACC) &  % partner feature
    0.21 (+) **** &  % point-biserial
    
    mMean\_avg (ACC) & % friends feature
    0.18 (+) **** % pearson
    
    
    \\
    
    &
    {dmListMin\_min (ACC)} & % family feature
    {0.17 (+) ****} &  % pearson
    
    {zAxisAvgMean\_avg (ACC)} &  % people feature
    {0.09 (+) ***} &  % pearson
    
    mMed\_avg (ACC) &  % partner feature
    0.21 (+) **** &  % point-biserial
    
    mSMAMean\_avg (ACC) & % friends feature
    0.19 (+) ****   % pearson
    
    
    \\
    
    
    
    &
    {angleYMin\_min (ACC)} & % family feature
    {0.17 (+) ****} &  % pearson
    
    {entertainment\_max (APP)} &  % people feature
    {0.09 (+) **} & % pearson
    
    mSMAMed_avg (ACC) &  % partner feature
    {{0.58 (+) ****}}&  % point-biserial
    
    yAxisAvgMin\_min (ACC) & % friends feature
    0.18 (-) **** % pearson
    
    
    \\
    
    &
    {mNewMin\_min (ACC)} & % family feature
    {0.16 (+) ***} &  % pearson
    
    {communication\_avg (APP)} &  % people feature
    {0.09 (+) ***} & % pearson
    
    mStd\_avg (ACC) &  % partner feature
    0.21 (+) ****&  % point-biserial
    
    xAxisAvgStd\_max (ACC) & % friends feature
    0.18 (+) **** % pearson
    
    \\
    
    &
    {mNewMed\_min (ACC)} & % family feature
    {0.16 (+) ***} &  % pearson
    
    {screen\_avg (SCR)} &  % people feature
    {0.09 (-) **}  &  % pearson
    
    mSMAStd\_avg (ACC) &  % partner feature
    0.21 (+) ****&  % point-biserial
    
    angleXStd\_max (ACC) & % friends feature
    0.18 (+) *** % pearson
    
    
    \\
    
    \rowcolor{red!5}
    &
    \textbf{Feature (Sensor)} & 
    \textbf{PCC} &
    -&
    -&
    \textbf{Feature (Sensor)} & 
    \textbf{PCC} &
    \textbf{Feature (Sensor)} &
    \textbf{PCC} 
    \\
    
    
    \multirow{10}{*}{\rotatebox[origin=c]{90}{\footnotesize{three-class}}}  &
    {angleXMed\_min (ACC)} & % family feature
    0.18 (+) **** &  % pearson
    
    - &  % people feature
    - &  % pearson
    
    mMean\_avg (ACC) &  % partner feature
    0.24 (+) **** &  % point-biserial
    
    mMean\_avg (ACC) & % friends feature
    {0.23} (+) **** % pearson
    \\
    
    
    &
    {angleXMax\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    - &  % people feature
    - & % pearson
    
    mSMAMean\_avg (ACC) &  % partner feature
    0.24 (+) **** &  % point-biserial
    
    mSMAMean\_avg (ACC) & % friends feature
    0.23 (+) ****   % pearson
    \\
    
    &
    {angleYAvg\_min (ACC)} & % family feature
    {0.18 (+) ****} &  % pearson
    
    - &  % people feature
    - &  % pearson
    
    mMed\_avg (ACC) &  % partner feature
    0.23 (+) **** &  % point-biserial
    
    yAxisAvgMin\_min (ACC) & % friends feature
    0.23 (-) ****   % pearson
    \\
    
    
    
    &
    {angleYMin\_min (ACC)} & % family feature
    {0.17 (+) ****} &  % pearson
    
    - &  % people feature
    - &  % pearson
    
    mSMAMed\_avg (ACC) &  % partner feature
    0.23 (+) ****&  % point-biserial
    
    mMean\_max (ACC) & % friends feature
    0.23 (+) ****  % pearson
    \\
    
    &
    {angleXMean\_min (ACC)} & % family feature
    {0.17 (+) ****} &  % pearson
    
    - &  % people feature
    - & % pearson
    
    mSMAMax\_avg (ACC) &  % partner feature
    0.23 (+) ****&  % point-biserial
    
    mSMAMean\_max (ACC) & % friends feature
    0.23 (+) ****  % pearson
    \\
    
    &
    {system\_min (APP)} & % family feature
    {0.17 (+) ****} &  % pearson
    
    - &  % people feature
    - & % pearson
    
    mMax\_avg (ACC) &  % partner feature
    0.23 (+) **** &  % point-biserial
    
    mMed\_avg (ACC) & % friends feature
    0.23 (+) **** % pearson
    \\
    
    &
    {dmListMin\_min (ACC)} & % family feature
    {0.17 (+) ***} &  % pearson
    
    - &  % people feature
    - &  % pearson
    
    mStd\_avg (ACC) &  % partner feature
    0.23 (+) **** &  % point-biserial
    
    mSMAMed\_avg (ACC) & % friends feature
    0.23 (+) ****   % pearson
    \\
    
    
    
    &
    {angleYMax\_min (ACC)} & % family feature
    {0.17 (+) ***} &  % pearson
    
    - &  % people feature
    - & % pearson
    
    mSMAStd_avg (ACC) &  % partner feature
    {{0.23 (+) ****}}&  % point-biserial
    
    mSMAMax\_avg (ACC) & % friends feature
    0.23 (+) **** % pearson
    \\
    
    &
    {mNewMin\_min (ACC)} & % family feature
    {0.16 (+) ***} &  % pearson
    
    - &  % people feature
    - & % pearson
    
    mMed\_max (ACC) &  % partner feature
    0.22 (+) ****&  % point-biserial
    
    mMax\_avg (ACC) & % friends feature
    0.23 (+) *** % pearson
    
    \\
    
    &
    {mNewMed\_min (ACC)} & % family feature
    {0.16 (+) ***} &  % pearson
    
    - &  % people feature
    -  &  % pearson
    
    mSMAMed\_max (ACC) &  % partner feature
    0.22 (+) ***&  % point-biserial
    
    dmListStd\_max (ACC) & % friends feature
    0.23 (+) *** % pearson
    
    \\
    
    \hline
    
    \end{tabular}}
    \label{tab:correlation}
    
\end{table}
